HighDist Framework: Algorithms and Applications

We introduce the problem of determining if the mode of the output distribution of a quantum circuit (given as a black-box) is larger than a given threshold, named HighDist, and a similar problem based on the absolute values of the amplitudes, named HighAmp. We design quantum algorithms for promised versions of these problems whose space complexities are logarithmic in the size of the domain of the distribution, but the query complexities are independent. Using these, we further design algorithms to estimate the largest probability and the largest amplitude among the output distribution of a quantum black-box. All of these allow us to improve the query complexity of a few recently studied problems, namely, $k$-distinctness and its gapped version, estimating the largest frequency in an array, estimating the min-entropy of a distribution, and the non-linearity of a Boolean function, in the $\tilde{O}(1)$-qubits scenario. The time-complexities of almost all of our algorithms have a small overhead over their query complexities making them efficiently implementable on currently available quantum backends.

==> approx-min.tex <==
\section{Algorithm for approximate minimum}\label{sec:approx-min}

In this section, we present a quantum algorithm to solve the approximate minimum finding problem.
The problem of approximate minimum finding can be stated as follows: given an $n$-size $m$-valued array $A$ as an oracle $O$ where $O$ acts as $O\ket{i}\ket{b} = \ket{i}\ket{b\oplus A[i]}$, an accuracy parameter $\epsilon$ and an error parameter $\delta$, output a valued $y$ such that $|y - \min_iA[i]| \le \epsilon$ with probability at least $1-\delta$.

\begin{algorithm}
    \caption{Algorithm for approximate minimum finding \label{algo:approx-min}}
    \begin{algorithmic}[1]
        \Require Oracle $O_D$ (with parameters $m$,  $a$), threshold $\tau$, accuracy $\epsilon$ and error $\delta$.
        \State Set $r=\log(m)+a$, $\tau' = \tau - \frac{\epsilon}{8}$, $q = \lceil \log(\frac{1}{\epsilon}) \rceil +4$ and $l= q+3$.
        \State Set $\tau_1 = \left\lfloor{\frac{2^l}{\pi}\sin^{-1}(\sqrt{\tau'})}\right\rfloor$
        \State Initialize $3$ registers $R_1R_2R_3$ as $\ket{0^\logn}\ket{0^\logn}\ket{\tau_1}$ and $\frac{1}{2(8/\pi^2 - 1/2)^2}$ many independent copies of $R^k_4 R^k_5 = \ket{0^l}\ket{0}$ .
        The $3^{rd}$ register is on $l$ qubits.
        \State {\bf Stage 1:} Apply $O_D$ on $R_1$ and $R_2$.
        \On{the $\frac{1}{2(8/\pi^2 - 1/2)^2}$ independent copies}
        % \State In $\log(\frac{1}{\delta\tau})$ many independent copies do:
            \State {\bf Stage 2:} Apply quantum amplitude estimation sans measurement ($AmpEst$) on
            $O_D$ with $R_2$ as the input register, $R^k_4$ as the precision register and 
            $R_1$ is used to determine the ``good state''. $AmpEst$ is called with 
            error at most $1- \frac{8}{\pi^2}$ and additive accuracy $\frac{1}{2^q}$.\label{line:amp_est}
            \State {\bf Stage 3:} Use ${\tt HD_l}$ on $R_3$ and $R^k_4$
            individually.\label{line:half_dist}
            \State {\bf Stage 4:} Use ${\tt CMP}$ on $R_3 = \ket{\tau_1}$ and $R^k_4$ as input registers 
            and $R^k_5$ as output register.\label{line:q_compare}
            \State {\bf Stage 3:} Use ${\tt HD^{\dagger}_l}$ on $R_3$ and $R^k_4$
            individually.\label{line:half_dist_inv}
        \EndOn
        \State Compute the majority of all the $R^k_5$ states and store it in a new register $R_f$.
        \State {\bf Stage 5:} Apply Amplitude Amplification 
        (AA) $O(\frac{1}{\sqrt{\tau}})$ times on $R_f$ with error at most $\delta/2$ 
        and measure $R_f$ as $out$.
        \State If $out = \ket{1}$ \Return{\tt TRUE} else \Return{\tt FALSE}\label{line:finish}
        % \If{$out = \ket{1}$}
        %     \State \Return {\tt TRUE}
        % \Else
        %     \State \Return {\tt FALSE}
        % \EndIf \label{line:finish}
    \end{algorithmic}
\end{algorithm}

==> conclusion.tex <==
\section{Conclusions}

{\color{red} to add}

We studied several problems in the low-space complexity regime by reducing them to two very generic problems which we call as \prob and \pmaxprob. Our algorithm for \prob can roughly determine if the probability of any outcome of a given quantum circuit is larger a specified threshold and that for \pmaxprob uses the earlier algorithm to approximate the largest probability among all its outcomes. These algorithms are then used to solve the $k$-distinctness of an $n$-sized array with $O(n^{3/2})$ query complexity, and estimate the \Finf of an $n$-sized array using $O((n/\epsilon)^{3/2} \log(n/\epsilon))$ queries, requiring only $O(\log n)$ qubits in both scenarios. Our algorithms are designed using amplitude amplification and estimation and their time-complexities have a small overhead over their query complexities.

% Apart from the efficient few-qubit algorithms for some common problems another impact of our work is the formal study of the reductions between them. The reduction not only allow efficient upper bounds on their complexities, but also obtaining lower bounds. 
% It should be possible to obtain lower bounds on the query complexities of the problems studied in this paper by reducing them from the {\tt $\Delta$-Approximate Count} problem studied by Nayak et al.~\cite{Nayak1999QuantumStatistics}. Other interesting directions

% It would be interesting to study the time-space tradeoffs of the above problems and design quantum algorithms in the streaming setting in which, apart from the number of qubits, the objective is to also minimize the number of passes over an input.

% Consider the k-distinctness problem. The reduction from the $k$-distinctness problem to sorting is very trivial; sort the $n$ inputs and check if there are $k$ consecutive indices in the sorted array with the same element.
% In a classical setting, the time-space tradeoff lower bound of element distinctness problem is closely tied with that of the sorting problem.
% Beame in~\cite{Beame1991AElements} showed a lower bound of $TS = \Omega(n^2)$ for sorting a list of $n$ numbers from the range $[1,n^2]$.
% In~\cite{Yao1994Near-OptimalDistinctness}, Yao showed a lower bound of $TS = \Omega(n^{2-\varepsilon(n)})$ where $\varepsilon(n) = O(1/(log(n))^{1/2})$ proving a conjecture first made by Borodin et al. in~\cite{Borodin1979AMachines}.
% So, classically the problem of element distinctness seems ``nearly" as hard as the problem of sorting.
% However, such a relation does not seem to hold in the quantum setting. A lower bound of $TS = \Omega(n^{3/2})$ was showed for sorting by Klauck in~\cite{Klauck2003QuantumSorting}.
% As for element distinctness, the quantum walk algorithm due to Ambainis has a complexity of $T = O(n/\sqrt{S})$ which for $S = \log(n)$ has the relation $TS = O(n/\log(n))$ which is strictly below $\Omega(n^{3/2})$.
% However, to the knowledge of the authors there does not exist any work on the time-space tradeoff lower bounds for the element distinctness or in general the $k$-distinctness problem.
% Moreover, it is quite fascinating to see two closely related problems of similar difficulty in classical setting when introduced in the quantum setting have strictly different levels of difficulty.

==> lowerbounds.tex <==
\section{Lower bounds}
\label{sec:lowerbounds}

For our lower bounds we reduce from the \countdec problem that takes as input a binary string of length $n$ and decides if the number of ones in $X$, denoted $|X|$, is $l_1$ or $l_2 > l_1$, given a promise that one of the two cases is true. We use the following lower bound on the query complexity of this problem that was proved by Nayak and Wu~\cite{Nayak1999QuantumStatistics}.


% Consider the following count decision problem: given a string $X\in\{0,1\}^n$ decide if $|X|=l_1$ or $|X|=l_2\neq l_1$ given a promise that one of the two cases is true.
% Mathematically, let $f_{l_1,l_2}$ be a partial function defined such that for any $X\in \{0,1\}^n$, $f_{l_1,l_2}(X) = 0$ if $|X|=l_1$ and $f_{l_1,l_2}(X) = 1$ if $|X|=l_2$.
% Then the count decision problem is the problem of evaluating the function $f_{l_1,l_2}$ on any given input $X\in\{0,1\}^n$.
% On the lines of evaluating $f_{l_1,l_2}$, Nayak and Wu in their work~\cite{Nayak1999QuantumStatistics} gave the following result:

\begin{theorem}[\countdec lower bound~\cite{Nayak1999QuantumStatistics}]\label{thm:nayak_wu}
Let $l_1, l_2 \in [n]$ be two integers such that $l_2 > l_1$, and $X$ be an $n$-bit binary string. Further, let $l_2 - l_1 = 2\Delta$ for some integer $\Delta$. Then any quantum algorithm takes $\Omega(\sqrt{n/\Delta} + \sqrt{(l_2-\Delta)(n-(l_2-\Delta))}/\Delta)$ queries to solve the \countdec problem.
\end{theorem}

% We first derive a lower bound for the \dgkd problem.

\begin{proof}[Lemma~\ref{lemma:dgkd-lb} (lower bound for \dgkd)]
Consider the following reduction from \countdec to \dgkd.
Let $X\in \{0,1\}^n$ be a given input string with the promise that either $|X|=\frac{n}{t}-2d$ or $|X|=\frac{n}{t}$ for some $t=O(1)$ and some $1\le d \le \frac{n}{2t}$. Theorem~\ref{thm:nayak_wu} states $\Omega(\tfrac{n}{d})$ queries are required to decide the value of $|X|$. 

Now, construct an array $A^X$ of size $n$ such that $A^X[i] = i$ if $X_i = 0$ and $A^X[i] = n+1$ if $X_i=1$.
For any $X$ such that $|X|=\frac{n}{t}-2d$, there are $\frac{n}{t}-2d$ many distinct indices of $A$ that have the same element $n+1$. Similarly, for any $X$ such that $|X|=\frac{n}{t}$, there are $\frac{n}{t}$ many distinct indices that have the same element. Therefore, any algorithm that decides the \dgkd problem with $k=\tfrac{n}{t}$ and $\Delta=2d$ also decides if $|X|=\frac{n}{t}-2d$ or $|X|=\frac{n}{t}$, and using Theorem~\ref{thm:nayak_wu}, we get that the quantum query complexity of the \dgkd problem is $\Omega(n/d) = \Omega(\frac{n}{\Delta})$.
\end{proof}

\begin{proof}[Lemma~\ref{lemma:finf-lb} (lower bound for \Finf)]
Consider the array $A^X$ that was constructed in proof of Lemma~\ref{lemma:dgkd-lb}. To decide whether $A^X$ has at least $\tfrac{n}{t}$ identical elements or no element appears more than $\tfrac{n}{t}-2\Delta$ times, it suffices to run any algorithm for \Finf on $A^X$ with additive accuracy $\Delta/2$. In the former case, the algorithm will return an estimate that is at least $\tfrac{n}{t}-\Delta/2$, and in the latter case, the algorithm will return an estimate that is at most $\tfrac{n}{t}-\tfrac{3}{2}\Delta$. Clearly, both the cases can be easily distinguished and so we obtain the desired lower bound for \Finf on $n$-sized arrays with $\Delta/2$ additive accuracy.
\end{proof}

Lemma~\ref{lemma:pmax-lb} follows from Lemma~\ref{lemma:finf-lb} since the \Finf problem can be trivially reduced to the \pmaxprob problem by scaling the accuracy parameter.

Proof of Lemma~\ref{lemma:highdist-lb} involves a reduction from the \countdec problem as well as application of the quantum adversary method. We have explained it in Appendix~\ref{sec:highdist-lb}.

% Notice in the proof that any string of Hamming weight $\frac{n}{t}$ for some integer $t\ge 2$, is reduced to an array of size $n$ with exactly $\frac{n}{t}+1$ distinct elements and similarly for an $X$ such that $|X| = \frac{n}{t}-2\Delta$.
% More generally, an input $X$ to count decision problem induces an $n$-sized $\big(|X|+1\big)$-valued array $A^{X}$ through reduction which is the input to the \dgkd problem.

% Next, we provide similar lower bounds to the the mode estimation problem, the \prob problem and the \pmaxprob problem.
% The reductions from \dgkd problem to \Finf estimation problem is quite trivial.
% Given an array $A$ as input to \dgkd problem, provide $A$ as the input to \Finf problem to estimate $f_{\infty}$ of $A$ with additive accuracy $\Delta/3$. If the output $\hat{f}_{\infty}\ge k-\frac{\Delta}{2}$, then output {\tt TRUE} else output {\tt FALSE}.
% This reduction leads to the following lemma.

% \begin{lemma}
% \label{lemma:finf_lower_bound}
% Any quantum algorithm that estimates \Finf with additive accuracy $\epsilon$ uses $\Omega(n/\epsilon)$ queries to the given array.
% \end{lemma}
% {\color{red}
% As for the \prob problem, a reduction from \dgkd problem to \prob problem is discussed in Section~\ref{sec:gkd}. Such a reduction yields the following lemma.

% \begin{lemma}
% \label{lemma:hd_lower_bound}
% Given an oracle that generates a distribution $D = (p_x)_{i=1}^n$, any quantum algorithm that solves the \promiseprob problem uses $\Omega(1/\epsilon)$ queries to the oracle.
% \end{lemma}

% Now, in any distribution $D=(p_x)_{i=1}^n$ and a threshold $\tau$, it is direct that if $p_{max} \ge \tau$ then there exists some $x\in [n]$ such that $p_x \ge \tau$ and if $p_{max}< \tau-\epsilon$ for some $\epsilon$ then for all $y\in [n]$ we have $p_y < \tau-\epsilon$.
% This informs that any algorithm that solves \pmaxprob problem also solves \prob problem. We have the following lemma as the consequence.

% \begin{lemma}
% \label{lemma:pmax_lower_bound}
% Given an oracle that generates a distribution $D = (p_x)_{i=1}^n$, any quantum algorithm that estimates \pmaxprob with additive accuracy $\epsilon$ uses $\Omega(1/\epsilon)$ queries to the oracle.
% \end{lemma}
% }
